Flash-Splat: 3D Reflection Removal with Flash Cues and Gaussian Splats

We introduce a simple yet effective approach for separating transmitted and reflected light. Our key insight is that the powerful novel view synthesis capabilities provided by modern inverse rendering methods (e.g.,~3D Gaussian splatting) allow one to perform flash/no-flash reflection separation using unpaired measurements -- this relaxation dramatically simplifies image acquisition over conventional paired flash/no-flash reflection separation methods. Through extensive real-world experiments, we demonstrate our method, Flash-Splat, accurately reconstructs both transmitted and reflected scenes in 3D. Our method outperforms existing 3D reflection separation methods, which do not leverage illumination control, by a large margin. Our project webpage is at https://flash-splat.github.io/.

==> figures/3_method_old.tex <==


\section{Method}
\label{sec:method}



\subsection{The Flash No-Flash Concept}

\input{figures/fig4_Overview}
\input{figures/fig4_pipeline}


Capturing a pair of flash and no flash images of a scene at the same camera viewpoint can be leveraged to reconstruct a reflection-free image. Reflections exist because objects in the reflected scene reflect light from ambient light sources. \mingyang{Because glass transmits much more than than it reflects, when one uses flash, only the transmission scene is illuminated. Hence, if one can measure a `flash-only' image one would have captured a reflection-free image.} In practice capturing a flash-only image $\mathbf{I}_{FO}$ is only possible in a pitch-dark environment, so one technique used among photographers is subtracting a flash image $\mathbf{I}_{F}$ from a no-flash image $\mathbf{R}_{NF}$~\cite{lei2021robust}:
\begin{align}
    \mathbf{I}_{NF} &= \beta_{NF}\mathbf{R}_{NF} + \mathbf{T}_{NF} \\
    \mathbf{I}_{F} &= \beta_{NF}\mathbf{R}_{NF} + \mathbf{T}_{NF} + \beta_{FO}\mathbf{R}_{FO} + \mathbf{T}_{FO} \\
    \mathbf{I}_{FO} &= \mathbf{I}_{F} - \mathbf{I}_{NF} = \beta_{FO}\mathbf{R}_{FO} + \mathbf{T}_{FO} \label{eqn:reflection_free}
\end{align}
where $\mathbf{T}$ is the transmission scene, $\mathbf{R}$ is the reflection scene and $\beta$ is the reflective fraction factor. \mingyang{Note that because glass reflects very little}, $\mathbf{R}_{FO}\approx 0$, so $\mathbf{I}_{FO}$ is effectively a reflection-free image. \autoref{fig:motivation} demonstrates how this process works.

Unfortunately, this process only works when you capture the flash-free and flash image at the exact same location and orientation. Any small movement results in misaligned images so the formulas no longer hold. Even vibrations due to sources such as pressing the shutter button or flash popup can cause removal errors even when using a tripod as shown in \autoref{fig:example_unpaired_2d}.


% \begin{itemize}
%     % \item Flash only math equation
%     % \item physics description of how flash helps
%     % \item Paired is key! fig showing what happens with unaligned images
%     % \item Description why this is a huge hindrance for practical cases. even with tripod, mismatch could be caused by pressing the camera button. so many sources of vibration
%     \item maybe move eq 3 up here
% \end{itemize}



% \subsection{Reflection Removal using Flash Cues}

% \subsection{Proposed GS Model Architecture}

% \input{figures/fig4_pipeline}

% \subsection{Flash Cue Prior Loss}

% \subsection{Flash aware point cloud init}
% \begin{itemize}
%   \item Fusing multi-view animations
%   \item Motion extraction and applying to source 360 image
% \end{itemize}



% \begin{figure*}[!t]
%   % \centering
%    \includegraphics[width=\textwidth]{sec/figs/network_architecture.png}
%    \caption{\textbf{Method Overview}. Inputs of 3D coordinates and ray direction are processed through Multi-Layer Perceptrons (MLPs) to predict transmission and reflection characteristics. The model essentially generates two separate NeRFs, one for the transmission scene, and the other for the reflection scene. In addition, it also has two additional MLP branches to output 2 weighting factors, where $\alpha$ and $\beta$ are the weights of the transmission scenes of the flash image and no flash image, respectively. 2 Loss functions are jointly minimized. Note that the difference of these two functions represents the key idea of this paper -- flash minus no flash equals a scaled version of the reflection-free transmission scene, which serves as a powerful prior for the reflection/transmission separation.}
%    \label{fig:method_overview}
% \end{figure*}

% \subsection{Flash / No Flash Photography}


% The technique of subtracting a "no flash" image from a "flash" image is not a new approach in image processing to address unwanted reflections introduced by a camera flash. In a typical scenario, the flash increases the brightness of the transmission scene, but maintains the same brightness of the reflected scenes coming from surfaces like glass or water. Subtracting the pixel values of the no-flash image from the flash image cancels out the reflected scene, but keeps the transmission scene brightened  by the flash. This method is employed to produce reflection-free, enhancing the overall quality and clarity of the captured scene, particularly in computational photography applications.

% To explain this in more detail, let us consider how the light rays of the flash interact with the scene. The flash emits light rays directed towards the scene, which engage with objects. When these rays encounter reflective surfaces, such as glass, they split into two components: some continue through the surface, while others bounce back. The light reflected from the glass or other reflective surfaces returns towards the camera. 

% When capturing a "flash image," it records both the light transmitted through the scene and the light reflected from it, including any unwanted reflections. Conversely, the "no flash image" captures the ambient light and pre-existing reflections but lacks the supplementary illumination from the flash. Subtracting the pixel values of the "no flash" image from the "flash" image effectively eliminates shared elements present in both images, encompassing ambient light and common reflections. What remains are the disparities, which often accentuate the flash's effects and can yield a cleaner image with reduced reflections. This computational technique proves especially advantageous in scenarios where reflections from surfaces like glass pose a challenge to achieving the desired quality in the captured photograph.

% \subsection{Flash / No Flash With NeRF}
% Naively, we can capture paired flash no flash images for each view, and then we take the difference for each pair to get the reflection free view, and the job is done. However, this is very troublesome, since it would require a tripod to capture paired images, which is not feasible for smart phone users or people who don't carry tripods. Fortunately, with the novel view synthesis ability of NeRF, we no longer need to capture paired data. Even with unpaired flash and no flash images, we can still interpolate between views using NeRF, and calculate "pseudo" paired flash / no flash views.

% Before we go into the details of our proposed method, we briefly recap the basics of NeRF. In NeRF, the scene is represented by a function \( F \) that maps a 5D vector of spatial coordinates and viewing directions to a color and density. The vector comprises 3D coordinates \((x, y, z)\) and 2D viewing directions \((\theta, \phi)\). The function \( F(x, y, z, \theta, \phi) \) outputs RGB color values and a volume density at each point.

% The rendering of a scene in NeRF involves calculating the color of light along camera rays. For a ray \( R \), the color \( C(R) \) is computed by integrating the contributions of all points \( p \) along the ray, weighted by their volume densities and the transmittance from the camera to point \( p \). Mathematically, this is represented as:
% \begin{align}
% \label{eqn:nerf}
% C(R) = \int_{t_n}^{t_f} T(t) \sigma(p) c(p) \, dt
% \end{align}
% % \[
% % \]

% where \( t_n \) and \( t_f \) are the near and far bounds of integration, \( T(t) \) is the transmittance function, \( \sigma(p) \) is the volume density, and \( c(p) \) is the color at point \( p \).



\subsection{Proposed Pipeline}

To make flash-no-flash based reflection removal practical, we introduce a novel unpaired technique. Our key idea is novel view synthesis enables a pseudo-pairing where instead of directly capturing corresponding flash and no flash images, one can simply render the missing view of the 3D reconstruction.
Our method pipeline is shown in Fig.~\ref{fig:pipeline}. 

% \topic{Problem formulation.}
% Similar to NeRFReN~\cite{guo2022nerfren}, the color $\mathbf{C}$ of a pixel is formulated as reflection-transmission composition using,
% \begin{equation}
%     \mathbf{C} = \mathbf{T} + \beta \mathbf{R} \,,
% \end{equation}
% where $\mathbf{T}$ is the color from transmissive component, $\mathbf{R}$ is the color from reflective component, and $\beta$ is a reflection fraction factor. 
% Our goal is to estimate $\mathbf{T}$, $\mathbf{R}$ and $\beta$ for each pixel in the rendering.

% \topic{Flash and non-flash images.}
% Our method leverages the flash as a physical cue to better decompose the transmissive component and the reflective component.
For a scene, we capture some viewpoints with flash and some others without flash.
Then, we aim to reconstruct a 3D representation of the captured flash and no-flash images.
We consider four 3D scenes in total: transmission with flash $\mathbf{T}_{F}$, transmission without flash $\mathbf{T}_{NF}$, reflection $\mathbf{R}$, and the reflective fraction factor $\beta$. 
To render a target pixel in a captured image, we blend the overlapping regions of the transmissive and reflective scenes.
We then have,
\begin{align}\label{eqn:pixel_values}
\begin{split}
    \mathbf{I}_{NF} &=  \mathbf{T}_{NF} + \beta \mathbf{R} \\
    \mathbf{I}_{F} &=  \mathbf{T}_{F} + \beta \mathbf{R} \,
\end{split}
\end{align}
for flash ($F$) images and no-flash ($NF$) images.
% By subtracting the equations above, we eliminate the reflection and have
% \begin{equation}
%     \mathbf{C}^{F} - \mathbf{C}^{NF} = (\beta^{F} - \beta^{NF})
% \end{equation}
We use a standard rendering procedure to calculate the pixel values in~\eqref{eqn:pixel_values}, and then compute a reflection-free image with~\eqref{eqn:reflection_free}.


% We consider two types of 3D Gaussians: transmissive part $G(\mathbf{x}^{t})$ and reflection part $G(\mathbf{x}^{r})$. 

% In addition to the original 3D Gaussian distributions $G(\mathbf{x})$, we also formulate the transmission fraction factor $\beta$ as a 1D Gaussian.

% In the proposed model, 3D coordinates and directional information of rays are fed into a series of Multi-Layer Perceptrons (MLPs). These MLPs are intricately designed to analyze and predict the distinct characteristics of both transmission and reflection components within a scene. Fundamentally, the model operates by creating two individual Neural Radiance Fields (NeRFs): one is dedicated to modeling the transmission scene, while the other focuses on capturing the reflection scene. This dual-NeRF approach allows for a more nuanced and accurate representation of the complexities involved in scenes with reflective surfaces.

% Beyond the basic scene reconstruction, the model is also adept at calculating and providing two essential weighting factors. These factors are represented by the variables \(\alpha\) and \(\beta\). Specifically, \(\alpha\) corresponds to the weight attributed to the transmission scene in the scenario where flash illumination is used, while \(\beta\) relates to the weight of the transmission scene captured without the use of flash. The introduction of these weighting factors is a crucial aspect of the model, as it allows for a more refined and controlled blending of the transmission scenes under varying illumination conditions, leading to more accurate and realistic scene reconstructions.

% \textcolor{blue}{NeRFReN paraphrase}

% Our proposed network architecture is inspired by the advances made in the field of Neural Radiance Fields (NeRF). The network is notably characterized by a tripartite multilayer perceptron (MLP) structure, each part fulfilling a distinct function in rendering realistic 3D scenes. This design enables the network to handle complex interactions of light within the scene with unprecedented detail and accuracy.

% The first MLP in the network is tailored for transmission. It focuses on modeling how light travels through and interacts with different materials within the scene. This component is crucial for accurately capturing effects like light scattering, transparency, and translucency, which are essential for rendering scenes where light interacts in complex ways with the environment.

% The second MLP is dedicated to reflection. Its role is to understand how light reflects off various surfaces, considering factors such as surface texture, material properties, and the angle of incidence. This MLP is key to realistically rendering reflective surfaces, ensuring that the objects in the scene interact with light in a believable manner.

% A smaller, yet vital third MLP in the network is tasked with modeling the relative weights between transmission and reflection. This MLP serves as an integrator, determining the extent to which the final image is influenced by either light transmission or reflection. It harmonizes the outputs from the transmission and reflection MLPs, resulting in a balanced and realistic composite. The inclusion of this third MLP distinguishes our network, enabling it to adeptly render scenes where the interplay between light transmission and reflection is intricate and nuanced.

% In summary, our network's unique architecture, comprising three specialized MLPs for transmission, reflection, and the balancing of these components, represents a significant advancement in computer graphics. This structure allows for the rendering of highly detailed and photorealistic 3D scenes, capturing the complex behaviors of light with a level of fidelity not seen in traditional models.



% \yiran{Are we still using the tricks below?}
% \subsubsection{Flash/No Flash Regularization}

% \subsection*{Problem Setup in NeRFReN}

% NeRFReN extends NeRF by introducing separate components for handling transmission and reflection. The total rendered image, or the composite, is a combination of these components.

% Let \( F_{trans}(x, y, z, \theta, \phi) \) and \( F_{refl}(x, y, z, \theta, \phi) \) be the functions modeled by the transmission and reflection MLPs, respectively. These functions output respective color and density values for transmission and reflection.

% The composite color \( C_{comp}(R) \) for a ray \( R \) is then a blend of the transmission and reflection contributions, weighted by a factor determined by the third MLP, denoted as \( w_{blend} \). The formula for the composite color is:


% \begin{align}
% \label{eqn:nerf}
% C_{noflash}(R) & = \alpha \cdot C_{trans}(R) + C_{refl}(R) \\
% C_{flash}(R) & = \beta \cdot C_{trans}(R) + C_{refl}(R)
% \end{align}

% % \[
% % \]

% where \( C_{trans}(R) \) and \( C_{refl}(R) \) are the colors calculated for transmission and reflection, respectively.
% \begin{align}
% \label{eqn:nerf}
% C_{noflash}(R) & = \alpha \cdot C_{trans}(R) + C_{refl}(R) \\
% C_{flash}(R) & = \beta \cdot C_{trans}(R) + C_{refl}(R)
% \end{align}


% In the method outlined by the equations, two different images are created to represent the scene with and without flash. The 'No Flash Image' is composed by taking the transmission of light through the scene, which is the light that isn't reflected, and multiplying it by a weight $\beta$. To this, the reflection component, which is the light bouncing off surfaces in the scene, is added. The equation for this is:

% \begin{equation}
% \text{No Flash Image} = \beta \times \text{Transmission} + \text{Reflection}
% \end{equation}


% \begin{align}
% \label{eqn:nerf}
% C_{noflash}(R) & = \alpha \cdot C_{trans}(R) + C_{refl}(R)
% \end{align}


% The 'Flash Image' is similarly constructed but uses a different weight, $\alpha$, for the transmission. The reflection component remains the same as in the no-flash case. The equation is:

% % \begin{equation}
% % \text{Flash Image} = \alpha \times \text{Transmission} + \text{Reflection}
% % \end{equation}

% \begin{align}
% \label{eqn:nerf}
% C_{flash}(R) & = \beta \cdot C_{trans}(R) + C_{refl}(R)
% \end{align}

% When we subtract the 'No Flash Image' from the 'Flash Image,' the reflection terms are identical in both and thus cancel out. The result is an image that represents only the transmission affected by the flash, scaled by the difference between $\alpha$ and $\beta$. The equation for this difference is:

% \begin{equation}
% \text{Flash Image} - \text{No Flash Image} = (\alpha - \beta) \times \text{Transmission}
% \end{equation}

% \sachin{This needs to be reworked with appropriate symbols}
% \begin{align}
% \label{eqn:nerf}
% C_{flash}(R) - C_{noflash}(R) = (\alpha - \beta) \cdot C_{trans}(R)
% \end{align}

% This resulting equation is significant because it cancels out the reflection scene. By examining this difference, one can understand how much more brightness the flash lighting contributes to the transmission scene, which is equivalent to taking a photo of the scene using a flash within a dark room. The resulted photo would be reflection free.

% \subsubsection{Additional Training Strategies}
% \textbf{Handling View Dependency. } We have 2 separate training stages with regard to view dependency. In the first stage, we don't use any view dependency in our training, as in, we assume both the reflection and transmission scenes are diffuse, and the only specular information comes from the planar reflection that we are trying to separate. This assumption significantly decrease the ill-posedness of the training, and make it much easier to separate transmission and reflection. After we separated the transmission and reflection, we go to the second training stage, where we add in view dependency of both scenes. This will further increase our rendering quality.\\
% \topic{Differentiable Raw Processing. } Our network is directly trained on raw data. We implemented a differential post processing pipeline to turn RAW data into postprocessed whitebalanced and tonemapped RGB images. The losses are all calculated in the postprocessed image space, which makes our rendering more realistic.\\
% \textbf{Smoothness Priors. } We also regularize the training by enforcing smoothness of the depths, which helps 

% max lowpass = 0.01 #0.01
% 我们理论上不会学反 reflection和transmission
% \yiran{Do we use other loss functions other than the ones in FSGS~\cite{zhu2023fsgs}?}

\subsection{3D Gaussian Splatting}
We chose a 3D representation where the scene is represented explicitly as a group of 3D Gaussians (3DGS)~\cite{kerbl20233dgs}. 
Each Gaussian consists of a position vector $\mathbf{\mu} \in \mathbb{R}^3$, a covariance matrix $\mathbf{\Sigma} \in \mathbb{R}^3$, opacity $o \in \mathbb{R}$ and appearance feature by $n$ spherical harmonic (SH) coefficients $\{\mathbf{c}_i \in \mathbb{R}^3 | i=1,2,\ldots,n \}$.
It corresponds with a 3D point $\mathbf{x}$ following the Gaussian distribution:
\begin{equation}
%    G(\mathbf{x}) = \frac{1}{(2\pi)^{3/2}|\mathbf{\Sigma}|^{1/2}} \exp{(-\frac{1}{2}(\mathbf{x}-\mathbf{\mu})^\top \mathbf{\Sigma}^{-1}(\mathbf{x}-\mathbf{\mu})  )}   \,.
    G(\mathbf{x}) = (2\pi)^{-3/2}|\mathbf{\Sigma}|^{-1/2} \exp\pare{-\frac{1}{2}(\mathbf{x}-\mathbf{\mu})^\top \mathbf{\Sigma}^{-1}(\mathbf{x}-\mathbf{\mu})  }   \,.
\end{equation}
% In addition, each Gaussian distribution stores an opacity $o \in \mathbb{R}$ and the appearance feature by $n$ spherical harmonic (SH) coefficients $\{\mathbf{c}_i \in \mathbb{R}^3 | i=1,2,\ldots,n \}$.
%where $n=D^2$ is the number of SH coefficients with degree $D$. 
For rendering, 3DGS blends all 3D Gaussians based on their opacity by projecting the 3D covariance matrix onto the camera coordinate system.
% \begin{equation}
%     \mathbf{c} = \sum_{i=1}^{n} \mathbf{c}_i \alpha_i \prod_{j=1}^{i-1} (1 - \alpha_j) \,,
% \end{equation}
% where $\alpha_i$ is computed from a 2D Gaussian with a covariance $\mathbf{\Sigma}^{\prime} \in \mathbb{R}^{2\times2}$ multiplied by the opacity $o$. $\mathbf{\Sigma}^\prime$ is computed as the projection of the 3D covariance matrix $\mathbf{\Sigma}$ onto the camera coordinate system:
% \begin{align}
%     \mathbf{\Sigma}^{\prime} = \mathbf{JW}\mathbf{\Sigma} \mathbf{W}^{\top} \mathbf{J}^{\top}
% \end{align}
% where $\mathbf{J}$ is the Jacobian of the affine approximation of the projection transformation and $\mathbf{W}$ is the view transformation matrix.
In practice, we build our pipeline upon FSGS~\cite{zhu2023fsgs}, a variant of 3DGS that supports feedforward settings. 


\subsection{Optimization objectives}
\topic{Raw data reconstruction loss.}
3DGS~\cite{kerbl20233dgs} computes $\mathcal{L}_1$ loss and SSIM loss between the captured RGB images and the rendered images.
However, we find that...
\yiran{Add some reasons why we use it here}.
We compute $\mathcal{L}_1$ loss and DSSIM loss~\cite{Baker:DSSIM} with the Gamma-corrected $\gamma(\cdot)$ raw images.
% Our new reconstruction loss is,
\begin{align}
    &\mathcal{L}_1 = \mathcal{L}_1\pare{\gamma\pare{\mathbf{I}^{raw}}, \gamma\pare{\gamma^{-1}\pare{\mathbf{T}} + \beta \gamma^{-1}\pare{\mathbf{R}}} }  \\
    &\mathcal{L}_{DSSIM} = \mathcal{L}_{DSSIM}\pare{\gamma\pare{\mathbf{I}^{raw}}, \gamma\pare{\gamma^{-1}\pare{\mathbf{T}} + \beta \gamma^{-1}\pare{\mathbf{R}} }}.
\end{align}

\topic{Flash/No-Flash linearity regularization.} From~\eqref{eqn:pixel_values}, we know the transmissive components of the flash image and no-flash image are linearly related --- as the only difference is the amount of light available to hit the camera sensor. 
We introduce a Pearson Correlation between two components. 
\begin{equation}
    \mathcal{L}_{corr} = \frac{\text{cov}\pare{\mathbf{T}_{NF},\mathbf{T}_{F}}}{\sqrt{\text{var}\pare{\mathbf{T}_{NF}}\text{var}\pare{\mathbf{T}_{F}}}}  
\end{equation}
\sachin{Can we explain why introducing a loss is better than a hard constraint? If they are perfectly linear, then $\alpha T_F=T_{NF}$ seems better. In practice, specular objects do not have this relationship, but that suggests we shouldn't even use this loss. If our method only works on diffuse scenes anyway, why give the model any room to learn non-diffuse relations? Can we claim learning ``some'' specular appearance? Also, I think it needs a better subscript than $corr$.}
% Incorporating the linearity as a loss instead of a hard constraint adds capacity to the 3D representation to learn 
% % section 3.3
% \begin{itemize}
%     % \item we turn to unpaired
%     % \item novel views help bc you can pretend you have that pair
%     \item explain pearson linearity, why hard constraint causes issues
% \end{itemize}

\topic{Final loss function.}
Our total loss function is:
\begin{equation}
    \mathcal{L} = \lambda_1 \mathcal{L}_1 + \lambda_2 \mathcal{L}_{DSSIM} + \lambda_3 \mathcal{L}_{corr} \,,
\end{equation}
where $\lambda_1, \lambda_2, \lambda_3$ are hyperparameters we tune.


% 


==> figures/fig11_glass_removal.tex <==
\begin{figure}[t!]
  % \centering
   \includegraphics[width=\columnwidth]{images/Fig_11_GlassRemoval.pdf}
   \caption{Pseudo GT.}
   \label{fig:glass_removal}
\end{figure}


==> figures/fig5_main_exp_test.tex <==
\begin{figure}[t!]
  % \centering
   \includegraphics[width=\columnwidth]{images/Fig_5_MainExp_Test.pdf}
   \caption{Comparison with NeRFReN~\cite{guo2022nerfren} and Dong et al.~\cite{dong2021location} on Outdoor Scenes. We include two additional reference images at the top. }
   \label{fig:compare_baselines_outdoor}
\end{figure}


==> figures/fig8_ablation_fnf.tex <==
\begin{figure}[t!]
  % \centering
   \includegraphics[width=\columnwidth]{images/Fig_8_Ablation_FnF.pdf}
   \caption{\textbf{Effectiveness of Linearity constraint $\mathcal{L}_{linearity}$ (Equation~\ref{eqn:linearity}).}
   With $\mathcal{L}_{linearity}$, both NeRFReN and Gaussian Splatting are improved.
   }
   \label{fig:abla_gs_nerf_lin}
\end{figure}

==> figures/fig9_ablation_raw.tex <==
\begin{figure}[t!]
  % \centering
   \includegraphics[width=\columnwidth]{images/Fig_9_Ablation_Raw.pdf}
   \caption{\textbf{Effectiveness of raw reconstruction loss (Equation~\ref{eqn:raw_loss}).}
   With raw reconstruction loss, the reflection and reflection depth become sharper.
   }
   \label{fig:raw_loss}
\end{figure}

==> figures/fig_rebuttal_1_SOTA.tex <==
% \begin{figure*}[th!]
%    \centering
%    \includegraphics[width=\textwidth]{images/00_RoughFig.pdf}
%    \caption{aaaaa}
%    \label{fig:overview}
% \end{figure*}


